Outlier-Robust Spatial Perception: Hardness, General-Purpose Algorithms, and Guarantees

Spatial perception is the backbone of many robotics applications, and spans a broad range of research problems, including localization and mapping, point cloud alignment, and relative pose estimation from camera images. Robust spatial perception is jeopardized by the presence of incorrect data association, and in general, outliers. Although techniques to handle outliers do exist, they can fail in unpredictable manners (e.g., RANSAC, robust estimators), or can have exponential runtime (e.g., branch-and-bound). In this paper, we advance the state of the art in outlier rejection by making three contributions. First, we show that even a simple linear instance of outlier rejection is inapproximable: in the worst-case one cannot design a quasi-polynomial time algorithm that computes an approximate solution efficiently. Our second contribution is to provide the first per-instance sub-optimality bounds to assess the approximation quality of a given outlier rejection outcome. Our third contribution is to propose a simple general-purpose algorithm, named adaptive trimming, to remove outliers. Our algorithm leverages recently-proposed global solvers that are able to solve outlier-free problems, and iteratively removes measurements with large errors. We demonstrate the proposed algorithm on three spatial perception problems: 3D registration, two-view geometry, and SLAM. The results show that our algorithm outperforms several state-of-the-art methods across applications while being a general-purpose method.

==> arXiv_supp_SLAM.tex <==
%!TEX root = supplemental.tex

\newpage
\clearpage
\subsection{Supplemental for Robust SLAM}
\label{sec:supp_slam}

\input{supp_fig-slam}

==> fig-alg.tex <==
%!TEX root = main.tex

\begin{figure}[t]
	\begin{center}
	\begin{minipage}{\textwidth}
	\hspace{-0.2cm}
	\includegraphics[width=.5\columnwidth]{FBT-exec} 
	\end{minipage}
\caption{Visualization of a few itarations of \name (see notation introduced in Section~\ref{sec:algorithms}).  At the beginning of each iteration, the forward step of \name builds a set $\selSet$ of seemingly outlying measurements.  It does so until the ``outlier-free'' performance bound $\perfBudgMin_{\grSet\setminus \selSet}$ is met (green, dashed line).  Then, the backward step of \name reinstates measurements in $\selSet$ as inliers.  It does so until the ``outlier-free'' bound is violated by an addititive factor $a(i)r(\emptyset)$ (orange, dotted line), during the $i$-th iteration. The process continuous until concensus is achieved.
	 \label{fig:FBT-exec}}
	\vspace{-8mm} 
	\end{center}
\end{figure}

==> supp_guarantees.tex <==
\section{Proof of Theorem~\ref{th:guarantees}}
\label{sec:supp_guarantees}

First observe that $\res^\star_{|\selSet|}\leq \res(\selSet)$.  This holds true due to the definition of $\res^\star_{|\selSet|}$ as the smallest value of $\res(\cdot)$ among all sets with cardinality $|\selSet|$. Next, define the quantities:
\begin{itemize}
	\item $f(\selSet)\doteq \res(\emptyset)-\res(\selSet)$;
	\item $f^\star\doteq \res(\emptyset)-\res^\star_{|\selSet|}$.
\end{itemize}
We observe that:
\begin{align*}
f^\star&= \res(\emptyset)-\res^\star_{|\selSet|}\\
&\leq \res(\emptyset)\\
&= \res(\emptyset)+\res(\selSet)-\res(\selSet)\\
&=f(\selSet)+\res(\selSet).
\end{align*}
The above now imples:
\begin{align*}
\frac{f(\selSet)}{f^\star}&\geq 1- \frac{\res(\selSet)}{f^\star} \\
&\geq 1- \frac{\res(\selSet)}{f(\selSet)},
\end{align*}
where the latter holds since $f(\selSet)\leq f^\star$, which in turns holds because $\res(\selSet)\geq \res^\star$.  Finally, the above is:
\begin{align*}
\frac{f(\selSet)}{f^\star}&\geq 1- \apost_\selSet,
\end{align*}
which gives:
\begin{align*}
\res(\emptyset)-\res(\selSet)&\geq (1- \apost_\selSet)\res(\emptyset)- (1- \apost_\selSet)\res^\star_{|\selSet|} \Rightarrow\\
\apost_\selSet(\res(\emptyset)-\res^\star_{|\selSet|})&\geq \res(\selSet)-\res^\star_{|\selSet|}
\end{align*}
which gives eq.~\eqref{eq:guarantees}.  

To prove eq.~\eqref{eq:bound_refined}, we first observe that $\res^\star\geq \res^\star_{|\selSet|}$, since $|\selSet| \geq |\selSet^\star|$.  Now, it can be verified that:
\begin{equation}\label{app:eq:aux_guarantees}
\frac{\res(\selSet)-\res^\star}{\res(\emptyset)-\res^\star}\leq \frac{\res(\selSet)-\res^\star_{|\selSet|}}{\res(\emptyset)-\res^\star_{|\selSet|}},
\end{equation}
since it also is $\res(\emptyset)\geq \res(\selSet)$.
Substituting eq.~\eqref{app:eq:aux_guarantees} in eq.~\eqref{eq:guarantees}, the proof of the theorem is now complete.
